Decoupling Magnitude and Phase Estimation with Deep ResUNet for Music Source Separation

Deep neural network based methods have been successfully applied to music source separation. They typically learn a mapping from a mixture spectrogram to a set of source spectrograms, all with magnitudes only. This approach has several limitations: 1) its incorrect phase reconstruction degrades the performance, 2) it limits the magnitude of masks between 0 and 1 while we observe that 22% of time-frequency bins have ideal ratio mask values of over~1 in a popular dataset, MUSDB18, 3) its potential on very deep architectures is under-explored. Our proposed system is designed to overcome these. First, we propose to estimate phases by estimating complex ideal ratio masks (cIRMs) where we decouple the estimation of cIRMs into magnitude and phase estimations. Second, we extend the separation method to effectively allow the magnitude of the mask to be larger than 1. Finally, we propose a residual UNet architecture with up to 143 layers. Our proposed system achieves a state-of-the-art MSS result on the MUSDB18 dataset, especially, a SDR of 8.98~dB on vocals, outperforming the previous best performance of 7.24~dB. The source code is available at: https://github.com/bytedance/music_source_separation

==> old.tex <==


Third, although previous CNN based MSS systems such as UNets achieve state-of-the-art performance, there is a lack of research on exploring deep architectures for MSS. In this work, we propose to extend UNets to deep residual UNets by designing residual UNet blocks. We show that by designing a network narrower but deeper, the MSS performance will significantly increase.

First, the phase estimation in MSS is a challenging problem. 


One feature of the spectrogram domain methods is that the phase estimation are usually not included. Usually, the phase of the mixture is used as the recovered the target spectrogram. There is a disadvantage of using this kind of method, is that the phase can be different between target and mixture. To tackle this problem, several methods have been proposed to predict phases, such as complex value neural networks, PHASEN, etc. However, the performance of predicting phases can be difficult, as phase is more sensitive to predict. Also, the time domain systems have not outperformed the spectrogram domain system. 

In this work, we show that the difficulty of predicting phases is caused from directly predicting phases are difficult. Therefore, we propose a delta phase method to predict the phase difference between mixture and targets instead of the original phases. Another difficult of phase prediction is that the phase and magnitude have different scales, therefore the trianing can be non-steady. Therefore, we propose to implicilty predict the real and imagniary part and calculate the delta phase from the real and imaginary parts. Then we propose an algorithm to calculate the delta phase. 

In addition to previous works, we show that the previous shallow UNet and convolutioanl architectures may lead to underperformance of the source separation system because the receptive field is not so large. Therefore, we propose a deep residual unet up to 143 layers and show that the performance will improve with the residual architecture for the music source separation problem. When the computation cost are the same, the performance can be improved when using ResNet architecture.


\section{DeltaPhase}
Previous works are limited to the methodology that only apply magnitude masks. However, there is a lack of research investigating the mask distribution of the source separation problem. The masks are denoted as 

\begin{equation} \label{mask}
\begin{split}
M = Y / X \\
= \frac{Y_{r} + i Y_{i}}{X_{r} + i X_{i}} \\
= \frac{Y_{r}X_{r} + Y_{i}X_{i} + i(Y_{i}X_{r} - Y_{r}X_{i})}{X_{r}^{2} + X_{i}^{2}}
\end{split}
\end{equation}

Considering the real and imaginary part, the masks can be denoted as 



\subsection{Upperbound of music source separation targets}

To begin with, we analyzed the upperbound of music source separation tasks. The targets we investigated include mixture, ideal binary mask (IBM), ideal ratio mask, complex IRM, etc. This allows us to know the upperbound of systems.

\subsection{Distribution of Mask points}
To analyze why there are performance gap between IBM and IRMs, we show the distirbution of mask points as follows. To begin with, we plot the masks of vocals, accompaniment, bass and drums in Fig. xxx. We show that the angle of masks are distrbuted equally, while only using ideal binary mask will lead to the 0 angle of prediciton. Therefore, predicting angles and complex masks are neccessary. On the other hand, we evaluate the magnitude masks.Convential methods will limit the scale of ideal ratio masks to a scale between -1 and 1. However, we observe that there are magnitudes that beyond this range. 

\subsection{Proposed scale method}

To tackle this problem, we propose several systems. the first system is to predict the magnitude directly:

\begin{equation} \label{mask}
mag = relu(x)
theta = ...
\end{equation}

The second strategy is that we can use a weight to balance the prediction:

We also propose an IBM classification task, that requires the system to train with predicting IBM. So that if magnitude is less than 1, then weight tend to use sigmoid as output. If magnitude is bigger than 1, then tend to use linear as output.

To tackle the problem that the phases are not estimated, we propose an delta phase algorithm. Instead of only predicting the magnitude, we also predict the real and imaginary part of signals as described in Fig. \ref{figs:framework}. We denote the 

\noindent We denote the angle of mixture as $ \Theta_{\text{mix}} $, and the angle of $ s $ as $ \Theta_{\text{tar}} $. Our system predicts the incremental of angle $ \Theta_{\Delta} $. So that $ \Theta_{\text{mix}} = \Theta_{\text{tar}} + \Theta_{\Delta} $. Then, we have:
\begin{equation} \label{eq1}
\begin{split}
\hat{S} &= |\hat{S}| e^{\angle j\Theta_{\text{tar}}} \\
&= |\hat{S}|(\text{cos} \Theta_{\text{tar}} + j \text{sin} \Theta_{\text{tar}}) \\
&= |\hat{S}|(cos (\Theta_{\text{tar}} + \Theta_{\Delta}) + j sin (\Theta_{\text{tar}} + \Theta_{\Delta})) \\
&= |\hat{S}|(cos \Theta_{\text{tar}} cos \Theta_{\Delta} - sin  \Theta_{\text{tar}} sin \Theta_{\Delta} + j sin \Theta_{\text{tar}} cos \Theta_{\Delta} + j cos\Theta_{\text{tar}} sin \Theta_{\Delta})
\end{split}
\end{equation}


Previous works mainly apply conventional UNet for the source separation task. However, those UNet has several limitations. 1) The convolutional layers are only a few, and can be underfitting to the sound classes. 2) The receptive field size is limited, so the performance of separation can be limited. 3) We argue that immediately apply the decoder after encoder layers may lead to underperformance of systems.

To solve this problem, we propose a deep residual UNet to solve this problem. To begin with, the ResUNet consists of several residual blocks. We denote the residual block as follows. In previous works, Unets are shallow but wide. We argue that this kind of architecture may lead to underperofmrance in music source separation, because the deep architectures are important for MSS. We denote the residual blocks as:

The system contains 6 encoder layers, 4 intermediate layers and 6 decoder layers. Each encoder layer consists of 4 residual blocks, where each residual block consists of 2 convolutional blocks that are described in in Fig. xxx. Briefely speaking, a BN, leaky relu function with leakage of 0.01, and a linear convolutional layer. The input of the whole system is a complex spectrogram, and then converted to linear magnitude. For music source separation, there are stereo two channels as input. And for output, there are 6 channels, where magnitude, real and imaginary channels are individual. 

A few changes from previous ResNet include as follows:

1) Intermediate layers. We show that the intermediate layers are important for mss, which are increases the receptive field. 

2) Transpose and pooling layers 

3) Arbitrary loss function that can be calcualted on the wave domain. 

Fig. \ref{fig:resunet} shows the entire ResUNet architecture. There are encoder blocks, intermeidate blocks and decoder blocks in the diagram. The encoder and decoder blocks are symmetric. The output of the decoder block includes a magnitude, a real and an imaginary part. Then, the loss functions are calculated on the top of the system. Fig. \ref{fig:resblocks} shows the residual blocks of the resnet architecture. We show that this kind of deep architecture is helpful for the MSS task.

Therefore, estimating cIRM includes estimating the real and imaginary parts of mask $ M $. Fig. \ref{fig:cIRM} shows the demonstration of source signal, noise signal and mixture. The mixture signal is $ X_{t,f} = S_{t, f} + N_{t, f} $. It can be shown that the prediction of $ s $ from $ x $ includes a scaling and a phase rotation operation. Because:

\begin{equation} \label{eq:mask}
\begin{split}
Y & = MX \\
& = |M||X|e^{j (\angle M + \angle X)}
\end{split}
\end{equation}

\noindent so that $ |M| $ is the magnitude scaling factor, and the angle of $ M $ is the phase shift factor. In this work, we propose to predict the mask $ M $ to achieve the MSS task, that is different previous works \cite{}.

\begin{table*}[t]
\centering
\caption{Baseline result of IS paradigm and ES paradigm}
\label{table:upper_bound}
\begin{tabular}{*{12}{c}}
 \toprule
 & Mixture & IBM & cIBM & IRM (0, 1) & IRM (0, inf) & cIRM 1 & cIRM 2 & cIRM 3 & cIRM 5 & cIRM 10 & cIRM (0, inf) \\
 \midrule
 vocals & -5.69 & 10.59 & 12.44 & 10.04 & 10.42 & 19.84 & 31.02 & 35.58 & 41.04 & 47.62  & 54.50 \\
 accompaniment & -5.68 & 16.10 & 17.75 & 15.31 & 15.97 & 26.54 & 37.62 & 42.28 & 47.33 & 53.51 & 60.63 \\
 bass & -6.36 & 7.17 & 8.21 & 6.05 & 6.07 & 17.99 & 27.88 & 32.38 & 37.86 & 44.30 & 54.12 \\
 drums & -4.30 & 8.75 & 11.17 & 8.03 & 8.61 & 19.10 & 30.38 & 34.81 & 39.91 & 46.45 & 56.08 \\
 other & -4.92 & 8.20 & 9.54 & 7.28 & 7.37 & 18.97 & 28.91 & 33.63 & 39.08 & 45.64 & 56.00 \\
 \bottomrule
\end{tabular}
\end{table*}



\noindent Different mask types we evaluate include IBM, IRM, cIRM, and limited bounded cIRM etc. Those masks have been adopted to different MSS systems in previous works. We evaluate SDRs of different instruments on the test set of the MUSDB18 dataset, including vocals, accompaniment, drums and other. To begin with, we evaluate using mixture as source separation results. 

Table \ref{table:upper_bound} shows that vocals, bass, drums and other have negative SDRs when using mixture as separation result. The mixture result is used as a baseline for comparing with other mask based systems. We show that the upper bound of vocals using IRM is 10.02, which is the upper bound of several previous MSS systems. Considering current MSS systems can achieve higher performance than 7.0 dB, this result indicates that phase information must be incorporated into the model to achieve better performance. For accompaniment, the upperbound of using IRM is 15.97 dB, and current MSS system has higher performance than 13 dB. For bass, drums and other, the upperbound of IRM are 6.07 dB, 8.61 dB and 7.37 dB respectively. To further improve the system performance, phase information are important.

When extending IRM to cIRM, Table \ref{table:upper_bound} shows that the upperbound of MSS systems increase. Many previous works limit the magnitude of cIRMs to a constant such as 1. This assumes that the mixture magnitude is always larger than sources. We show that when limiting the magnitude of masks to 1, the upper bound SDR is 19.84 dB, which has a big gap to 54.50 dB, indicating that there are room for improvement. Table \ref{table:upper_bound} shows that the upperbound increase from 19.84 dB, to 31.02 dB, 41.04 dB, 47.62 dB and 54.50 dB when setting the mask magnitude to 1, 2, 5, 10, +inf, respectively. For other instruments such as accompaniment, bass, drums and other, the upperbound SDR increases significantly from IRM to cRIM, and also further increases when not limiting the magnitude of masks.


Previous IRM based methods assume that the angles between mixture and target source is unchanged. This is equavilent to that the angle is all 0. Fig. \ref{fig:cIRMs} shows the cIRMs distribution of vocals, accompaniment, bass, drums and other instruments. There are several T-F units that is beyond the -1 and 1 circle, indicating that limiting the mask magnitude to 1 will limit the MSS performance. There are more T-F units that have mask magnitudes larger than 1. Fig. \ref{fig:cIRMs} show that the cIRM distribution of different instruments are different. The angles distribute equally in all angles. We calculate how many TF bins have mask values larger than 1, and counted that 20.3\%, 34.5\%, 6.1\%, 26.9\% and 13.9\% TF bins have mask values larger than 1. This observation indicates that the cIRMs should be designed to have magnitudes larger than 1. 

To begin with, we denote the magnitude of the estimated mask as $ | \hat{M}_{\text{mag}} | \in [0, \infty)^{T \times F} $. Predicting the unbound mask $ | \hat{M}_{\text{mag}} | $ can be difficult. Following previous works, we can limit the magnitude of masks to $ (0, 1) $ by applying a sigmoid nonlinearity. Table \ref{table:upper_bound} shows the upper bound results of MSS systems by limiting different magnitudes of masks. After calculating the magnitudes, we calculate the phases of $ \hat{M} $ as follows. The neural network outputs $ \hat{P}_{\text{r}} \in \mathbb{R}^{T \times F} $ and $ \hat{P}_{\text{r}} \in \mathbb{R}^{T \times F} $ to calculate the phases of $ \hat{M} $ by:



In addition, the estimation of $ \hat{P_{\text{r}}} $ and $ \hat{P_{\text{}}} $ decouples the estimation of magnitude and phase. In total, a neural network contains three outputs: $ \hat{M} $, $ \hat{P_{\text{r}}} $ and $ \hat{P_{\text{}}} $ to calculate the cIRM of a source to be separated. The real and imaginary parts of the cIRM is calculated by:

contains both magnitude and angle information that should be applied on the mixture complex STFT. Then, we apply (\ref{eq:cIRM}) to calculate the complex STFT of the source to be separated. That is, we estimate the magnitude and phases of target source simultaneously instead of using the phase of mixture.


\noindent where $ \angle \hat{M} $ is calculated by (\ref{eq:cos_sin}).

Previous works have shown that directly estimate the linear spectrogram of $ \hat{S}_{\text{mag}} $ is difficult. Therefore, previous works will instead limit $ \hat{S}_{\text{mag}} $ by a sigmoid or a tanh non-linearity. We have shown that limiting the magnitude of $ \hat{S}_{\text{mag}} $ will have a upper bound of the system performance. Therefore, in this part we propose a combination of mask based and linear based method by introducing a weight function. The motivation is that the mask is used to be the main part of the separation system, and the linear magnitude is used to recover the residual part of the system.

The above equation shows that we are adding residual parts to the mask parts. This will break the upperbound of limiting the mask between -1 and 1. There are also other methods that can be used to extend the IRM upperbound. Our desing is to let $ a $ to control how much the system should attend to the mask, and how much it should attend to the linear part.

, still, there are many spaces to improve. First, previous UNet architectures are limited to tens of layers, which tend to underfit the training data. There is a lack of research on exploring deeper architectures for MSS. Second, the receptive field sizes of shallower CNNs are limited, and the global information on the spectrogram can not be captured. For example, shallower CNNs can not capture higher and lower frequency correlations on the spectrogram. 

In this work, we propose a deep residual UNet architecture for MSS. Different from previous UNet architectures, our proposed system contains hundreds of convolutional layers. We describe the residual UNet architecture as follows. To begin with, the waveform of an input mixture is converted into a spectrogram. Then, we apply batch normalization \cite{ioffe2015batch} on each frequency bins of the spectrogram to normalize input features. First, we build a conventional UNet for comparison. The UNet consists of 6 encoder and 6 decoder layers. Each encoder layer consists of two convolutional layers and a downsampling layer. Each decoder layer consists of a transposed convolutional layer for upsampling and two convolutional layers. Finally, three extra convolutional layers are added after decoder layers. In total, there are 33 layers in our UNet architecture.


========================

Conventional MSS systems are designed to separate a recording into vocals and accompaniments. Recently, MSS systems are designed to separate a recording into multiple instruments, such as vocals, bass, drums and other.

The coefficient $ A \in {0, 1}^{T \times F} $ is a learnable weight, which works as an attention submodule that controls how much a neural network should attend to $ |\hat{M}_{\text{mag}}||X| $, and how much it should attend to $ |\hat{P}| $. Larger $ A $ indicates that masks are more important for separation, and smaller $ A $ indicates that the linear spectrogram $ \hat{P} $ are more important for separation.


\begin{table}[t]
\centering
\caption{Baseline result of IS paradigm and ES paradigm}
\label{table:is_baseline}
\begin{tabular}{*{6}{c}}
 \toprule
 & vocals & bass & drums & other & accompaniment \\
 \midrule
 IRM oracle & 9.43 & 7.12 & 8.45 & 7.85 & - \\
 \midrule
 Open-Unmix \cite{stoter2019open} & 6.32 & 5.23 & 5.73 & 4.02 & - \\
 Wave-U-Net \cite{stoller2018wave} & 3.25 & 3.21 & 4.22 & 2.25 & - \\
 Demucs \cite{defossez2019music} & 6.29 & 5.83 & 6.08 & 4.12 & - \\
 Conv-Tasnet \cite{luo2019conv} & 6.81 & 5.66 & 6.08 & 4.37 & - \\
 splitter \cite{hennequin2020spleeter} & 6.86 & 5.51 & 6.71 & 4.55 \\
 D3Net \cite{takahashi2020d3net} & 7.24 & 5.25 & 7.01 & 4.53 & 13.52 \\
 Real Imag & 7.08 \\
 complex spectral mapping \cite{tan2019complex} & 7.05 \\
 DCCRN \cite{hu2020dccrn} \\
 phase-aware (withdraw) \cite{choi2020phase} \\
 phasen \cite{yin2020phasen} \\
 \midrule
 UNet & 7.20 & 4.16 & 6.14 & 4.62 \\
 UNetComplex & 7.52 \\
 \bottomrule
\end{tabular}
\end{table}



\begin{table*}[t]
\centering
\caption{Baseline result of IS paradigm and ES paradigm}
\label{table:is_baseline}
\begin{tabular}{*{6}{c}}
 \toprule
 & vocals & bass & drums & other & accompaniment \\
 \midrule
 UNet & 7.20 (22) & 4.79 (45) & 5.94 (45b) & 4.49 (45c) & 14.69 (51) \\
 UNetPhase \cite{choi2018phase} & 7.45 (37) & 5.42 (_47) & 6.51 (_47b) & 4.86 (_47c) & 15.23 (51b) \\
 UNetDecouple & 7.65 (39) & 5.00 (42) & 6.29 (42b) & 4.71 (42c) & 15.21 (51c) \\
 UNetComplex24 weight & 7.63 (38) & 5.50 (46) & 6.43 (46b) & 4.72 (46c) & 15.35 (51d) \\
 UNetDecouple+ &  7.81 (58) & 5.28 (58b) & 6.47 (58d) & 5.00 (58e) & 15.32 (58b) \\
 \midrule
 ResUNet & 7.79 (52) & 5.00 (55) & 6.20 (56) & 5.13 (57) & 16.15 (54) \\
 ResUNetDecouple & 8.72 (52b) & 5.71 (55b) & 6.50 (56b) & 5.20 (57b) & 16.39 (54b) \\
 ResUNetDecoupe+ & \textbf{8.98} (52c) & \textbf{6.04} (55c) & \textbf{6.62} (56c) & \textbf{5.29} (57c) & \textbf{16.63} (54c) \\
 \bottomrule
\end{tabular}
\end{table*}


The first system we compare is a conventional UNet. Then, we compare with several real and imaginary models, and also systems by predicting the phases directly. For fair comparisons with previous methods, we re-implemented many several previous systems including the unet based systems. Therefore, we can only replace several important parts of the system\st{,} and remain all other parts unchanged for fair comparison. 

\subsection{Comparison with residual architecture}
We investigate the residual unet with conventional unet architectures. We show that the residual architecture is indeed helpful for predicting the inversed spectrograms. After the neural network is deep enough, we are able to predict the separated spectrogram with high resolution. 

\subsection{Visualizing the cRIMS}
Fig. \ref{} shows the visualized predicted cIRMs. Comparing with the ground truth masks, we show that the magnitude can break the upper bound of 1. 

The limitation of this work is as follows. Although we proposed a framework that can achieve arbitrary upper bound of systems, however, there are still many spaces for improvement. For example, the estimated signals are still xx \% that do not overcome the limit 1. This indicates the estimating signals from mixture that has larger values are different tasks. 


We showed that the predicting of phases is important for source separation and there is an performance gap between using magnitudes with phases and using only magnitudes. We show that by decoupling the prediction of magnitudes and phases, we can achieve better results in MSS than several previous methods. We analyzed the distribution of complex ideal ratio masks (cIRMs). We proposed to combine mask and spectrogram-based methods for magnitude estimation to increase the performance upper bounds of music source separation (MSS) systems. We showed deep architectures are important for MSS and proposed a residual UNet with 143 layers that significantly outperforms shallower UNets. In future, we will explore to combine time-domain and time-frequency domain methods for MSS.


\begin{table}[t]
\centering
\caption{Comparison of SDRs of previous and our proposed MSS systems.}
\label{table:previous}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{*{6}{c}}
 \toprule
 & vocals & bass & drums & other & acc. \\
 \midrule
 IRM oracle & 9.43 & 7.12 & 8.45 & 7.85 & - \\
 \midrule
 Open-Unmix \cite{stoter2019open} & 6.32 & 5.23 & 5.73 & 4.02 & - \\
 Wave-U-Net \cite{stoller2018wave} & 3.25 & 3.21 & 4.22 & 2.25 & - \\
 Demucs \cite{defossez2019music} & 6.29 & 5.83 & 6.08 & 4.12 & - \\
 Conv-Tasnet \cite{luo2019conv} & 6.81 & 5.66 & 6.08 & 4.37 & - \\
 Spleeter \cite{hennequin2020spleeter} & 6.86 & 5.51 & 6.71 & 4.55 \\
 D3Net \cite{takahashi2020d3net} & 7.24 & 5.25 & \textbf{7.01} & 4.53 & 13.52 \\
 \midrule
 ResUNetDecouple+ & \textbf{8.98} & \textbf{6.04} & 6.62 & \textbf{5.29} & \textbf{16.63} \\
 \bottomrule
\end{tabular}}
\end{table}
